Transcription Methods for Trajectory Optimization: a beginners tutorial

This report is an introduction to transcription methods for trajectory optimization techniques. The first few sections describe the two classes of transcription methods (shooting \& simultaneous) that are used to convert the trajectory optimization problem into a general constrained optimization form. The middle of the report discusses a few extensions to the basic methods, including how to deal with hybrid systems (such as walking robots). The final section goes over a variety of implementation details.

==> tex/abstract.tex <==

\begin{abstract}
Multiple shooting is a common way to solve a trajectory optimization problem. This document is an overview of the practical details that have helped me implement multiple shooting algorithms. Once a trajectory optimization problem has been posed using multiple shooting, it can then be passed to a nonlinear optimization package, such as SNOPT or FMINCON. The suggestions in this document are based on experience, not rigerous experiments. If something doesn't quite make sense then you should test it yourself (and let me know if you find anything interesting!).
\end{abstract}

==> tex/collocation.tex <==
\section{Collocation Methods}

Collocation methods are based representing the optimal trajectory as a polynomial. Polynomials are nice because they can accurately represent nearly any smooth function, and their derivatives and integrals are easy to compute. This is useful because we can match the derivative of the polynomial approximation of the solution with the system dynamics at points along the trajectory. If they are identical, then the trajectory is feasible (at least as far as the dynamics are concerned). This is convenient, because it is often faster than running simulations, particularly if the dynamics are expensive to compute. Collocation can also be more accurate, assuming that the underlying solution is smooth and continuous. In addition, if orthogonal polynomials are used properly, the Jacobian of these derivative matching constraints is sparse.

\subsection{A more technical description}

 Let's assume that the system dynamics are given by:

\begin{equation} \label{eq:SystemDynamics}
\dot{\mathbf{x}} = f\left( t,\mathbf{x} \right)
\end{equation}

Now let's suppose that you represent the solution (soon to be optimal trajectory) as a $n^{th}$ order polynomial:

\begin{equation} \label{eq:PolynomialFunction}
\mathbf{x} = \mathbf{p}(t)
\end{equation}

In multiple shooting, the feasibility of the trajectory was ensured by breaking it up into many segments. Each trajectory was then stitched together using defect constraints that compared the state at the end of one segment to the state at the start of the next. This required running a simulation of each trajectory segments. In collocation, there is no simulation step. Rather, the system dynamics are satisfied by a constraint on the derivative of the solution at special grid points $t_i$:

\begin{equation} \label{eq:collocationDefects}
\mathbf{0} = \dot{\mathbf{p}}(t_i) - f\left( t_i,\mathbf{p}(t_i)  \right)
\end{equation}

If $\mathbf{p}$ is a $n^{th}$-order polynomial, then there are $n+1$ special grid points, whose spacing is determined by which class of orthogonal polynomial is being used\footnote{Using orthogonal polynomials is not required. The methods described in the following section are technically {\em orthogonal collocation methods}.}. For a Chebyshev polynomial \footnotemark{, these points are given by Equation \ref{eq:chebyshevPoints}, assuming that the domain of the trajectory has been scaled to the domain $[-1,1]$.

\begin{equation} \label{eq:chebyshevPoints}
t_i = \cos(i\pi/n), \quad i=0\dots n
\end{equation}

\footnotetext{There are similar equations for other orthogonal polynomials, but for simplicity, the following discussion will use the example of Chebyshev Polynomials, relying largely on the book: {\em ``Approximation Theory and Approximation Practice''} by Lloyd N. Tregethen \ADDREF{Trefethen}. }

The whole collocation method is based on representing polynomials using their values at each of these `special points'. Interestingly, this representation is analogous to representing a signal in the frequency domain (ie. taking its Fourier Transform), hence the alternate name for these techniques: {\em pseudo-spectral methods}. This makes it easy for the optimization algorithm to move around each point independently of the rest (the Jacobian of the constraints is sparse).

\par One nice property of storing a polynomial in this way is that its derivative is is easily calculated at each of these points. This makes calculating equation \ref{eq:collocationDefects} quite fast. A related property is that taking the integral of an orthogonal polynomial is incredibly easy - it is just a weighted sum of each coefficient (the polynomial's value at the special points). This is particularily useful for accurately computing integral cost functions, such as total work done by a motor.

\par Each special point has a basis function associated with it. The polynomial's value at an arbitrary point in the domain is calculated by taking a weighted average of these basis functions. This is called Barycentric Interpolation, and is shown in Equation \ref{eq:BarycentricInterpolation}. Note that $\lambda_i$ is pre-calculated based on the type of orthogonal polynomial.

\begin{equation} \label{eq:BarycentricInterpolation}
\mathbf{p}(\mathbf{x}) = \frac{
\sum_{i=0}^{n} \frac{\lambda_j \mathbf{p_j}}{\mathbf{x}-\mathbf{x}_j}
}{
\sum_{i=0}^{n} \frac{\lambda_j}{\mathbf{x}-\mathbf{x}_j}
}
\end{equation}

\subsection{Extensions of Collocation}

One of the limitations to the collocation methods described above is that they only work if the true solution is well-approximated by a polynomial. This is a good approximation for smooth dynamical systems, but once constraints are added, it is likely that the true solution will be discontinuous. One trivial example is swinging up a simple pendulum using a motor with restrictive torque limits. The optimal solution (by some cost functions) is to alternate between maximum torque in each direction. This solution is poorly captured by even a high-order polynomial.

\par The solution to this problem is to break up the trajectory into segments, in a similar manner to multiple shooting. The methods are very similar, except that the collocation version uses the same derivative matching constraints as above within each trajectory segment, where as the multiple shooting version uses a simulation. The trajectory segments are stitched together for the state variables (using defects like multiple shooting), but the control variable is allowed to be discontinuous.

\par The above fix is pretty good, but it has a problem: where to put the breaks between segments? As a first guess, the user can run multiple iterations of the algorithm with different spacings, but this is tedious and prone to error. A better method has been developed by Rao et al \cite{PattersonHagerRao}, which automatically breaks up the trajectory into the correct number of segments. Their method is called a {\em ``hp-adaptive''} scheme. It runs several iterations of the solver, and adaptively re-meshes the trajectory after each run. The breakpoints between trajectory segments are adjusted, as well as the order of the polynomial within each segment. Their full transcription algorithm is commercially available, under the name GPOPS II \cite{Rao_GPOPS_II} which will be discussed in a later section.




==> tex/constraints.tex <==
\subsection{Constraints}

In many trajectory optimization problems, there are constraints on the trajectory. It should be noted that these are different than a simple bound on the system input or state. In walking robots, common constraints are: 

\begin{itemize}
	\item reaction forces in friction cone
	\item robot above the ground
	\item robot moving forward
	\item foot hits ground from above... 
\end{itemize}

The most important thing to notice about constraints is that they must also be consistent and smooth. It isn't enough to say ``The lowest point of the foot during the step must be above the ground'' because this will pass data from a different grid-point on each function call. Rather, you need to say ``Every point of the foot trajectory must be above the ground'' (or use some very fancy smoothing in your maximization function). All rules that apply to objective functions regarding smoothness and consistency, also should be applied to calculations of constraints.

\par It is also important to minimize the number of unused constraints, provided that the problem remains smooth and consistent. One way to do this is to leave all of the constraints active, and then as you refine the solution, remove the constraints that are not being actively used. At the end of each run, check to make sure that the solution still satisfies the constraints.



==> tex/dataStructures.tex <==
\section{Data Structures}

I've found that one of the biggest sources for mistakes in writing trajectory optimization code is in collecting all of the various parts of the problem into a generic form that can be passed to a standard nonlinear optimization package. SNOPT requires that the decision variables be passed as a vector, and FMINCON requires that they be passed as a matrix (or vector/scalar). For multiple shooting, there are often several different types of decision variables, which are not simple to write as a matrix/vector. Consider a trajectory optimization to find the optimal walking trajectory for the Cornell Ranger (using a piecewise linear discritization of the controls):

\begin{itemize} \setlength{\itemsep}{0pt}

	\item{\bf Single Stance States - } [8 x N] matrix
	\item{\bf Single Stance Input - } [2 x (N+1)] matrix
	\item{\bf Single Stance Duration - } scalar
	\item{\bf Double Stance States - } [12 x M] matrix
	\item{\bf Double Stance Input - } [3 x (M+1)] matrix
	\item{\bf Single Stance States - } scalar

\end{itemize}

I've found that the best thing to do is to store each of these items as a single field in a struct (using Matlab for now). I then pass this struct to a special function that returns a new data structure that contains the field names, the order of the fields, and the size of each field. This function also returns all of the data from the struct collapsed into a single vector. This function is designed to work in both ways, so that calling it using a vector of data and the struct of field information will return a struct of data.

\par By writing a conversion function, between data struct and data vector, I can write all of the multiple shooting code using the data struct, and then just do a conversion before and after each interaction with the optimization algorithm. This makes all of the code that you write more readable, because you never have to reference a value using it's index in a vector. 

\par The program GPOPS takes this organization scheme to a new level by doing the struct to vector conversion itself, so you only ever work with the named variables in a struct.


==> tex/defects.tex <==
\subsection {Defects}

The whole idea behind multiple shooting is to take a complicated trajectory and break it into many simple trajectories. Each of these simple trajectories can then be adjusted nearly independently of the rest of the trajectory. Each trajectory section is connected to its neighbors using a {\it defect constraint}. Starting from any grid-point along a candidate trajectory, it is possible to integrate the system dynamics forward one step. The system state after this integration can then be compared with the state according to the candidate trajectory. The difference between these two state vectors is called a defect, and the defect constraint is used to tell the optimization algorithm to make all defects equal to zero. In math:

\begin{align}
	&\text{Trajectory}  &\{x_k,u_k\} \\
	&\text{Physics}  &\hat{x}_{k+1} = f(x_k,u_k,k) \\
  	&\text{Defect}  &d_k = \hat{x}_k - x_k
\end{align}

\par This becomes slightly more difficult to implement when there are hybrid dynamics, but the math is still fundamentally the same. Suppose that you want to find a trajectory for a walking system that has two continuous phases (single-stance and double-stance) and two switching events (heel-strike and toe-off). Let's suppose that you decide to give roughly 80\% of the time to single-stance and use 100 grid-points. In this case we get: 

\begin{align}
	&f( \cdot, \cdot, \{1..79\})  & \text{single-stance dynamics} \\
	&f( \cdot, \cdot, 80)  & \text{heel-strike map} \\
	&f( \cdot, \cdot, \{81-99\})  & \text{double-stance dynamics} \\
	&f( \cdot, \cdot, \{100\})  & \text{toe-off map} \\
\end{align}

\par Note here that our math would have a problem because there is no element before $1$ or after $100$. If the trajectory does not need to be periodic, then the solution is to only compute the defects for steps $1-99$. If the trajectory is periodic, then simply allow $k$ to wrap back around to $1$ after it reaches its maximum value.


==> tex/dynamics.tex <==
\subsection {Dynamics}

In order to get good convergence and accuracy, it is necessary that any discontinuities in the dynamics are lined up with a discontinuity in your discritization. For example, if there is a collision in the dynamics, then the problem should be broken up into two different sections: before the collision and after the collision. These two sections should then be constrained together by the discrete impact map for the collision. Another example would the that grid-points for a piecewise linear representation must line up with the grid-points used by the integration algorithm. Failure to do these things will cause failure to converge (or very slow convergence), and inaccuracy in the result.

\par Sometimes there are discontinuities hiding in `continuous' dynamics. Two common examples are the absolute value function and a saturation function, both of which have discontinuities in the first derivative. It is too cumbersome to line up grid-points with these sort of things, so the preferred method of dealing with them is to smooth them out. Examples for these smoothing functions are given in the source code for the Hammer Example, discussed at the end of the report. This sort of discontinuity are particularly problematic when the optimal trajectory lies near the discontinuity, such as trying to minimize $abs(x)$.

\par If there are hybrid dynamics, then it is good to let the optimization algorithm pick the duration of each continuous section of the trajectory. Note that the number of midpoints assigned to each continuous section must be constant throughout the optimization. This means that you must know the order and rough duration of the continuous phases of motion a priori. This is no longer a problem if your algorithm can use iterative grid refinement, although this makes the significantly more complicated.

==> tex/integrationAlgorithm.tex <==
\subsection{Integration Algorithm}

The integration algorithm is dependent on the discritization of your trajectory. If you are using a piecewise linear (or piecewise constant) representation, then the best method is to use a fixed step method, such as Euler integration or $4^th$ order Runge Kutta. Typically is it sufficient to have one integration step per grid-point, but there is no real harm in taking more steps (it will tend to increase accuracy of the dynamics, but increase computational time). 

\begin{itemize}
	\item{\bf Variable-Step vs. Fixed-Step: } It turns out that it is almost always better to use a fixed-step method when doing multiple shooting. This is because fixed-step methods are very consistent. This consistency is what helps make the optimization algorithm converge quickly. While variable-step methods might be more accurate, they lack in consistency. 

	\item{\bf High-Order vs. Low-Order: } There is some evidence that suggests that one $N^{th}$ order step is better than $N$ first order steps. It probably does not make a difference whether you use many low-order steps or few high-order steps. If searching for a very accurate solution it may be better to use a high-order method, but this address only one of several sources of error in resulting optimal trajectory.

	\item{\bf Error Checking: } Since it is not easy to know the accuracy of a fixed-step method, it is possible to check by comparing the final solution against a new simulation that uses a high-accuracy variable-step method. Integrate each section of the trajectory in series, using the final state of one section as the initial state in the next. If everything worked, the resulting trajectory should be a close match to the solution. Any errors that do appear will be compounded by the integration over the duration of the trajectory.

	\item{\bf Number of Substeps: } If $N_{Int}$ is too small, then there can be large errors in the integration, if $N_{Int}$ is too large, then the integration takes a long time. Given a fixed $N_u$ and $N_{Int}$, convergence rate increased as $N_x$ varied from $1$ (Single Shooting)  through $N_u$ (Collocation). As $N_x$ increases beyond $N_u$ the convergence does not improve and the runtime and memory requirements both increase. 

\par If you decide to use a pseudo-spectral method, then it is best to do the integration implicitly. This is done by implicitly integrating the underlying analytic function, using a weighted sum of the function value at each of the grid-points.

\end{itemize}


==> tex/introduction.tex <==
\section{Introduction}

The goal of trajectory optimization is to find a trajectory (system states and control as a function of time) that minimizes (or maximizes) some cost functional, usually subject to some set of constraints. This report will focus on finding optimal trajectories for continuous (or hybrid) dynamical systems. Much of the difficulty in solving a trajectory optimization problem is converting the continuous trajectory into a series of discrete constraints that a general purpose optimization algorithm can solve. This process is called transcription.

\par One of the best references for learning about this topic is: 

 ``Practical Methods for Optimal Control and Estimation Using Nonlinear Programming'' \cite{JohnT.Betts2001}. 
 
 Another good reference, somewhat more brief, is a paper by Diehl {\em et al.} \cite{Diehl2009}. \ADDSUB{Reference to Russ Tedrake's underactuated robot lectures}.

\subsection{Method Overview}

The most straight-forward way to solve a trajectory optimization is single shooting. Imagine that you are trying to hit a target using a canon. Single shooting is analogous to firing the canon several times, applying a small correction after each shot until you finally hit the target. This is a good method for simple problems, but it rapidly becomes infeasible for even moderately complicated problems.

\par Multiple shooting is a fairly simple improvement on single shooting. Instead of running on big simulation on each iteration, it breaks the trajectory up into many segments, and runs one simulation per segment. Now, in addition to hitting the target, a new set of constraints are added to force all of the segments to line up with each other. These new constraints are called defect constraints. It turns out that multiple shooting is a huge improvement on single shooting. If implemented properly, nearly all trajectory optimization problems can be solved with this method. 

\par Collocation methods are perhaps the most sophisticated way to solve trajectory optimization problems. They are similar to multiple shooting, but there is no numerical simulation of the trajectory over each segment. Instead, The trajectory is stored as an orthogonal polynomial. A feasibly solution is ensured by matching the derivative at special points along the trajectory to the system dynamics.

\subsection{Theorem: }
\begin{quote}
  {\em If there is a flaw in the problem formulation, the optimization algorithm will find it.}\footnote{The proof is left to the student}\cite{JohnT.Betts2001}
\end{quote}

==> tex/multipleShooting.tex <==
\section{Multiple Shooting Methods}

Multiple shooting is a transcription method for trajectory optimization. It works by breaking the desired trajectory up into a large number of segments. The transcription algorithm then runs an independent simulation for each segment. The feasibility of the trajectory (with respect to the system dynamics) is ensured by a {\em defect} constraint which requires the initial state of each trajectory segment to match the final state of the previous segment. 

\par This is a huge improvement over the more intuitive single shooting method, as shown in Figure \ref{fig:multipleShooting}. The key difference is that in multiple shooting there are many small defects (rather than one large defect). This makes the Jacobian of the defect constraints with respect to the control sparse and nearly linear, both of which dramatically improve the performance of the underlying optimization program.


\begin{figure} 
    \centering 
    \includegraphics[width = \columnwidth]{img/multipleShooting.pdf}    
    \caption{Solving the problem of moving a particle across a vector field. Notice how the multiple shooting produces several small defect vectors, and the single shooting produces one large defect vector. Also notice how the vector field influences the locations that the point passes through, allowing the trajectory to be drawn far from the initial guess.}     
    \label{fig:multipleShooting}     
\end{figure} 


\subsection{Integration Algorithm} \label{sec:IntegrationAlgorithm}

Each segment of the trajectory in the multiple shooting algorithm is calculated by running an explicit simulation. There are a wide variety of methods for computing this simulation, some of which are better than others.

\par In general it is better to have many short segments, rather than a few long segments. In general, the system should be well approximated by a linear model over the duration of each trajectory segment. For a quick approximate solution, a low order integration method such as Euler's method is good. For accurate trajectory, it is best to use a high-order method, such as $4^{th}$ order Runge-Kutta.

\par It is always preferable to use a fixed-step integrator, rather than a variable-step integrator. This is because fixed-step methods are consistent, where as variable-step methods accurate (but not consistent). The variable-step integrator is no consistent because a small change in an input (state or control) could change the number or relative size of integration steps, thus causing a discontinuity in the output across multiple iterations of the optimization algorithm. Consistency is required by the optimization algorithm for the gradients to accurate. A variable step method might make each individual simulation more accurate, but at the expense of the entire trajectory not converging properly. For the same reason, it is important to use an explicit integration method, to avoid an iterative solve that will be present in an implicit method.

\par One problem with a fixed-step explicit integration algorithm is that it is difficult to know the accuracy of the trajectory. This can have a negative effect on the trajectory as a whole, so it is always good to check the optimal trajectory that is returned from the optimization algorithm. A simple check is to take the system and run an open-loop simulation using a high-order variable-step integration algorithm, starting from the same initial conditions and using the same control actions as the optimal trajectory. The resulting trajectory can then be compared to the optimal trajectory - they should be reasonably close, although diverging exponentially in time.



==> tex/objectiveFunction.tex <==
\subsection{Objective Function}

The objective function must be smooth and consistent. This basically means that at any point, the linearizion of the system must be a good local approximation. Practically speaking, this means that absolute value function and functions that return the maximum value of a set are absolutely forbidden. There are a few ways to get around this restriction. One option is to directly smooth the function (such as arctangent smoothing), another is to introduce extra variables and constraints, which is more complicated, but nearly exact and better for convergence. Here is an example from Bett's book \cite{betts2010practical}:

\begin{align}
	& \text{BAD: } & |x| &	\\

	& \text{GOOD: } &  min(x_1+x_2) & \quad

 \text{subject to} \quad 
  \begin{cases}
	x=x_1-x_2 \\
	x_1>=0 \\ 
	x_2>=0	
  \end{cases}

\end{align}

%\begin{figure} 
%    \centering 
%    \includegraphics[width = \columnwidth]{img/fancyAbsValue.pdf}    
%    \caption{A fancy way to deal with absolute value functions}     
%    \label{fig:fancyAbsValue}     
%\end{figure} 

\par One commonly used objective function is to use the integral of the input squared against time. This has nice smoothness and consistency problems, and is vaguely related to things that people care about in real life. If an optimization problem is not converging, then it is usually a good idea to test it with a objective function of this form.

\par Another objective function, that is used in walking robotics applications, is Cost of Transport(CoT). This is typically more challenging to implement, but is directly related to real life. Smoothing is often required to use CoT in an optimization. CoT is also difficult for the optimization algorithm because it has a term for work, which typically is a product of some state and some actuator, making it very nonlinear.

%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Integral Objective Functions}

Many objective functions have a term in them that is the integral of some continuous function. While it may be tempting to use a simple integration scheme (such as one that just sums all of the values at the grid-points), this can cause problems. The best plan is to use the same integration algorithm for you dynamics and cost function. Practically, this amounts to creating a fake `state' to represent your integrand, and then passing it through the integration algorithm. This can be awkward to implement, but it is worth it. 


